Extremal Problems on Forest Cuts and Acyclic Neighborhoods in Sparse Graphs

Chernyshev, Rauch, and Rautenbach proved that every connected graph on $n$ vertices with less than $\frac{11}{5}n-\frac{18}{5}$ edges has a vertex cut that induces a forest, and conjectured that the same remains true if the graph has less than $3n-6$ edges. We improve their result by proving that every connected graph on $n$ vertices with less than $\frac{9}{4}n$ edges has a vertex cut that induces a forest. We also study weaker versions of the problem that might lead to an improvement on the bound obtained.

==> Figures/grid.tex <==
% \node() [] at (0,-2) {};
% \node() [] at (0,6) {};
% \node() [] at (4,-2) {};
% \node() [] at (4,6) {};
